Speckle Image Restoration without Clean Data

Speckle noise is an inherent disturbance in coherent imaging systems such as digital holography, synthetic aperture radar, optical coherence tomography, or ultrasound systems. These systems usually produce only single observation per view angle of the same interest object, imposing the difficulty to leverage the statistic among observations. We propose a novel image restoration algorithm that can perform speckle noise removal without clean data and does not require multiple noisy observations in the same view angle. Our proposed method can also be applied to the situation without knowing the noise distribution as prior. We demonstrate our method is especially well-suited for spectral images by first validating on the synthetic dataset, and also applied on real-world digital holography samples. The results are superior in both quantitative measurement and visual inspection compared to several widely applied baselines. Our method even shows promising results across different speckle noise strengths, without the clean data needed.

==> sec/9_rebuttal.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=1\textwidth]{img/psnr_result_1.png}
    \includegraphics[width=1\textwidth]{img/psnr_result_2.png}
    \caption{PSNR evaluations of all classes in the COIL-100 dataset. The PSNR measurements between noisy observations and restored images are computed. The differences are also shown by the line plot.}
    \label{fig:all_coil100_test}
\end{figure*}

\setcounter{section}{0}
\newpage
\section{Response to Reviewer 1 (\#9535)}
We thank reviewer 1 for the insightful suggestions and found our results convincing. We appreciate the reviewer also providing the writing suggestion and have revised the paper accordingly.

\subsection{\textbf{Performance evaluation on COIL-100.}}
We thank the reviewer for caring about the evaluation process used in this paper. To clarify, we demonstrated 6 different object classes drawn from a total of 100 classes in the COIL dataset. Each class we conducted in the 80\% / 20\% split for training (58 of 72 images) and testing (14 of 72 images), and reported the averaged score over the test set as described in Sec~\ref{sec:synthesized_dataset}. The images shown in Fig~\ref{fig:coil} are randomly drawn from the test split for visualization inspection. Note each object class is trained independently and evaluated using the same process applied for different classes and compared baselines.

In the main paper, the 6 representative classes are selected to demonstrate the capability of our proposed method can handle on different granularity of structures and patterns (also see in Sec~\ref{sec:synthesized_dataset}). In Figure~\ref{fig:all_coil100_test} of this rebuttal document, we provided the complete evaluation over the all 100 classes to show that the 6 classes are not just selected from the best outcomes. The results computed from the whole COIL-100 dataset shows our proposed algorithm can effectively denoise from averaged 20.68 PSNR of noisy observations, improving to averaged 36.77 PSNR, which is +16.09 PSNR improvement.

In our newly uploaded supplementary material, we included Figure~\ref{fig:all_coil100_test} as the reference for the further interested readers.

\subsection{\textbf{The term noise usually does not get plural. So correct
noises to noise.}}
Thanks for the revised suggestion. We have corrected the corresponding sentences in the revised paper.


\section{Response to Reviewer 3 (\#9539)}
We greatly appreciate reviewer 3 for the positive feedback and constructive suggestions. For each of the raised points, we address below individually:

\subsection{\textbf{The statement in page 1 seems not correct, multiplicative noise is essentially
the same one as additive noise after a logarithmic
transformation on pixel intensities.}}

We thank the reviewer for pointing out the last sentence in the third paragraph of page 1 is not strict, we are glad to revise it to \textit{"However, these denoisers are under the assumption about the noise is conditionally independent to the signal, which greatly degrades their performance when applied to coherent systems with multiplicative signal dependent noise."}. To further clarify, The additive and multiplicative noise we discussed in this paper is about how the noise effects on the signals (see \eqref{eq:additive} and ${\bf m}$ in \eqref{eq:multiplicative}), which is, whether the noise strength depends on pixel intensity.

In addition, although the logarithmic transformation can transform the multiplication into addition, we would like to highlight that the logarithmic transformation also forces us to deal with unbounded log space signals with one-sided negative infinity. i.e., log([0, 1]) into (-inf, 0]. The noise distribution and the corruption may be difficult to tackle in log space by neural networks. 


Consider the most of the noisy images obtained from optical devices are consists of both additive and multiplicative part, our proposed algorithm is able to deal with both kinds of noise, which can be further confirmed by the results shown in Sec~\ref{sec:dice_exp} about the real-world dice holography denoising. 

\subsection{\textbf{Computation complexity.}}
We agree with the reviewer that computation complexity is important in practical applications. We have calculated the total FLOPS needs for inference our proposed architecture (see Table~\ref{tab:model}), which is 17.35 GFLOPs, and also append this information at the bottom of Table~\ref{tab:model} in the revised paper. Although our architecture leverages ResUNet as the encoder, any encoder model can be adopted as it is deemed fit.









